IPPON: Common Sense Guided Informative Path Planning for Object Goal Navigation

Navigating efficiently to an object in an unexplored environment is a critical skill for general-purpose intelligent robots. Recent approaches to this object goal navigation problem have embraced a modular strategy, integrating classical exploration algorithms-notably frontier exploration-with a learned semantic mapping/exploration module. This paper introduces a novel informative path planning and 3D object probability mapping approach. The mapping module computes the probability of the object of interest through semantic segmentation and a Bayes filter. Additionally, it stores probabilities for common objects, which semantically guides the exploration based on common sense priors from a large language model. The planner terminates when the current viewpoint captures enough voxels identified with high confidence as the object of interest. Although our planner follows a zero-shot approach, it achieves state-of-the-art performance as measured by the Success weighted by Path Length (SPL) and Soft SPL in the Habitat ObjectNav Challenge 2023, outperforming other works by more than 20%. Furthermore, we validate its effectiveness on real robots. Project webpage: https://ippon-paper.github.io/

==> evaluation_result.tex <==
\begin{wraptable}{l}{.48\textwidth}
  \vspace{-1em}
    \begin{footnotesize} % This will apply the small font size to everything within the braces
    \centering
    \begin{tabular}{l*{3}{c}}
    \toprule
    Method & SPL  $\uparrow$ & SSPL  $\uparrow$ & SR $\uparrow$ \\
    
    \midrule
    
    Host team & 0.05 & 0.27 & 0.12 \\
    
    \rowcolor{Gray}
    
    Auxiliary RL~\cite{ye2021auxiliary} & 0.10 & 0.31 & 0.18 \\
    ICanFly & 0.26 & 0.37 & 0.43  \\

    \rowcolor{Gray}
    SkillFusion~\cite{staroverov2023skill} & 0.28 & 0.34 & 0.53 \\
    SkillTron~\cite{zemskova2024interactive} & 0.28 & 0.36 &  \textbf{0.59} \\

    \midrule

    IPPON (ours) & \textbf{0.34} & \textbf{0.46} & 0.54 \\

    \bottomrule
    \end{tabular}
  \caption{Evaluation results on the Habitat ObjectNav 2023 Challenge (standard phase). SR stands for the success rate.}
  \label{tab:object2023-evaluation}
  \end{footnotesize} % This will apply the small font size to everything within the braces
  \vspace{-1em}
\end{wraptable}
